ProteinWeaver: A Divide-and-Assembly Approach for Protein Backbone Design

Nature creates diverse proteins through a 'divide and assembly' strategy. Inspired by this idea, we introduce ProteinWeaver, a two-stage framework for protein backbone design. Our method first generates individual protein domains and then employs an SE(3) diffusion model to flexibly assemble these domains. A key challenge lies in the assembling step, given the complex and rugged nature of the inter-domain interaction landscape. To address this challenge, we employ preference alignment to discern complex relationships between structure and interaction landscapes through comparative analysis of generated samples. Comprehensive experiments demonstrate that ProteinWeaver: (1) generates high-quality, novel protein backbones through versatile domain assembly; (2) outperforms RFdiffusion, the current state-of-the-art in backbone design, by 13\% and 39\% for long-chain proteins; (3) shows the potential for cooperative function design through illustrative case studies. To sum up, by introducing a `divide-and-assembly' paradigm, ProteinWeaver advances protein engineering and opens new avenues for functional protein design.

==> tabs/table1-3.tex <==
\scalebox{0.5}{
\begin{tabular}{|c|clll|ccll|}
\hline
 &
  \multicolumn{4}{c|}{length200} &
  \multicolumn{4}{c|}{length400} \\ \hline
\multicolumn{1}{|l|}{} &
  \multicolumn{2}{c|}{quality} &
  \multicolumn{1}{l|}{novelty} &
  diversity &
  \multicolumn{2}{c|}{quality} &
  \multicolumn{1}{l|}{novelty} &
  diversity \\ \hline
 &
  \multicolumn{1}{c|}{scTM} &
  \multicolumn{1}{c|}{scRMSD} &
  \multicolumn{1}{l|}{Max TM} &
  Max Clust &
  \multicolumn{1}{c|}{scTM} &
  \multicolumn{1}{c|}{scRMSD} &
  \multicolumn{1}{l|}{Max TM} &
  Max Clust \\ \hline
PDB &
  \multicolumn{1}{c|}{0.974±0.075} &
  \multicolumn{1}{l|}{0.674±1.367} &
  \multicolumn{1}{l|}{--} &
  0.79 &
  \multicolumn{1}{c|}{0.969±0.155} &
  \multicolumn{1}{c|}{1.085±5.818} &
  \multicolumn{1}{l|}{--} &
  0.84 \\ \hline
RFDiffusion &
  \multicolumn{1}{c|}{0.982±0.103} &
  \multicolumn{1}{c|}{0.617±1.767} &
  \multicolumn{1}{l|}{0.6381±0.0075} &
  0.64 &
  \multicolumn{1}{c|}{0.927±0.155} &
  \multicolumn{1}{c|}{2.116±3.849} &
  \multicolumn{1}{l|}{0.6335±0.0045} &
  0.72 \\ \hline
Chroma &
  \multicolumn{1}{c|}{0.892±0.096} &
  \multicolumn{1}{c|}{1.776±1.532} &
  \multicolumn{1}{l|}{0.6738±0.0062} &
  0.62 &
  \multicolumn{1}{c|}{0.761±0.155} &
  \multicolumn{1}{c|}{4.891±4.489} &
  \multicolumn{1}{l|}{0.6262±0.0084} &
  0.95 \\ \hline
FrameFlow &
  \multicolumn{1}{c|}{0.953±0.114} &
  \multicolumn{1}{c|}{1.023±1.779} &
  \multicolumn{1}{l|}{0.6481±0.0099} &
  0.8 &
  \multicolumn{1}{c|}{0.805±0.190} &
  \multicolumn{1}{c|}{4.456±3.759} &
  \multicolumn{1}{l|}{0.6202±0.0078} &
  0.93 \\ \hline
FrameDiff (Latest) &
  \multicolumn{1}{c|}{0.893±0.104} &
  \multicolumn{1}{c|}{1.789±1.788} &
  \multicolumn{1}{l|}{0.6886±0.0053} &
  0.26 &
  \multicolumn{1}{c|}{0.799±0.168} &
  \multicolumn{1}{c|}{4.324±4.725} &
  \multicolumn{1}{l|}{0.6683±0.0060} &
  0.33 \\ \hline
ProteinWeaver &
  \multicolumn{1}{l|}{0.880±0.159} &
  \multicolumn{1}{l|}{--} &
  \multicolumn{1}{l|}{--} &
  -- &
  \multicolumn{1}{l|}{0.815±0.131} &
  \multicolumn{1}{l|}{--} &
  \multicolumn{1}{l|}{--} &
  -- \\ \hline
ProteinWeaver-sft &
  \multicolumn{1}{l|}{0.894±0.144} &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{l|}{--} &
  -- &
  \multicolumn{1}{l|}{0.805±0.132} &
  \multicolumn{1}{l|}{--} &
  \multicolumn{1}{l|}{--} &
  -- \\ \hline
ProteinWeaver-sppo &
  \multicolumn{1}{l|}{0.893±0.179} &
  \multicolumn{1}{l|}{1.7756±1.5322} &
  \multicolumn{1}{l|}{--} &
  -- &
  \multicolumn{1}{l|}{0.813±0.122} &
  \multicolumn{1}{l|}{4.4557±3.8492} &
  \multicolumn{1}{l|}{--} &
  -- \\ \hline
ProteinWeaver-sppo (bo3) &
  \multicolumn{1}{l|}{0.945±0.127} &
  \multicolumn{1}{l|}{1.459±1.798} &
  \multicolumn{1}{l|}{--} &
  -- &
  \multicolumn{1}{l|}{0.904±0.136} &
  \multicolumn{1}{l|}{2.187±3.549} &
  \multicolumn{1}{l|}{--} &
  -- \\ \hline
\end{tabular}
}

==> tabs/table3.tex <==
\begin{table}[t]
\footnotesize
\centering\setlength{\tabcolsep}{2pt}
\caption{Performance of ProteinWeaver on backbone design models evaluated using long chain lengths of 600 to 800. The reported results are the median±std of repetitive experiments.}
\label{tab:figure3}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccc|ccccc}
\toprule

&
  \multicolumn{5}{c}{\textbf{length600}} &
  \multicolumn{5}{c}{\textbf{length800}} \\

\cmidrule(lr){2-6} \cmidrule(lr){7-11}
 &
  \multicolumn{3}{c}{\textbf{Quality}} &
  \multicolumn{1}{c}{\textbf{Novelty}} &
  \textbf{Diversity} &
  \multicolumn{3}{c}{\textbf{Quality}} &
  \multicolumn{1}{c}{\textbf{Novelty}} &
  \textbf{Diversity} \\ 
 
 \cmidrule(lr){2-6} \cmidrule(lr){7-11}

 &
  \multicolumn{1}{c}{\textbf{scTM ↑}} &
  \multicolumn{1}{c}{\textbf{scRMSD ↓}} &
  \multicolumn{1}{c}{\textbf{Interface scTM ↑}} &
  \multicolumn{1}{c}{\textbf{Max TM ↓}} &
  \textbf{Max Clust ↑} &
  \multicolumn{1}{c}{\textbf{scTM ↑}} &
  \multicolumn{1}{c}{\textbf{scRMSD ↓}} &
  \multicolumn{1}{c}{\textbf{Interface scTM ↑}} &
  \multicolumn{1}{c}{\textbf{Max TM ↓}} &
  \textbf{Max Clust ↑} \\ 
  
\midrule
\rowcolor{gray!15} 
Native PDB &
  \multicolumn{1}{c}{0.94±0.07} &
  \multicolumn{1}{c}{2.03±2.33} &
  \multicolumn{1}{c}{0.95±0.05} &
  \multicolumn{1}{c}{--} &
  0.77 &
  \multicolumn{1}{c}{0.92±0.11} &
  \multicolumn{1}{c}{2.96±3.47} &
  \multicolumn{1}{c}{0.95±0.07} &
  \multicolumn{1}{c}{--} &
  0.8 \\ \hline
RFDiffusion &
  \multicolumn{1}{c}{0.66±0.19} &
  \multicolumn{1}{c}{9.95±5.68} &
  \multicolumn{1}{c}{0.73±0.15} &
  \multicolumn{1}{c}{\pmb{0.67±0.05}} &
  0.99 &
  \multicolumn{1}{c}{0.49±0.12} &
  \multicolumn{1}{c}{16.80±4.48} &
  \multicolumn{1}{c}{0.60±0.10} &
  \multicolumn{1}{c}{\pmb{0.66±0.06}} &
  \pmb{1.00} \\ \hline
Chroma &
  \multicolumn{1}{c}{0.62±0.17} &
  \multicolumn{1}{c}{11.40±5.91} &
  \multicolumn{1}{c}{0.69±0.13} &
  \multicolumn{1}{c}{\pmb{0.67±0.06}} &
  \pmb{1.00} &
  \multicolumn{1}{c}{0.62±0.14} &
  \multicolumn{1}{c}{12.75±6.13} &
  \multicolumn{1}{c}{0.67±0.11} &
  \multicolumn{1}{c}{0.68±0.07} &
  \pmb{1.00} \\ \hline
FrameFlow &
  \multicolumn{1}{c}{0.49±0.14} &
  \multicolumn{1}{c}{15.82±5.02} &
  \multicolumn{1}{c}{0.65±0.13} &
  \multicolumn{1}{c}{0.69±0.03} &
  \pmb{1.00} &
  \multicolumn{1}{c}{0.35±0.06} &
  \multicolumn{1}{c}{23.17±2.55} &
  \multicolumn{1}{c}{0.52±0.05} &
  \multicolumn{1}{c}{0.71±0.02} &
  \pmb{1.00} \\ \hline
FrameDiff &
  \multicolumn{1}{c}{0.45±0.08} &
  \multicolumn{1}{c}{16.19±3.35} &
  \multicolumn{1}{c}{0.57±0.06} &
  \multicolumn{1}{c}{0.72±0.03} &
  \pmb{1.00} &
  \multicolumn{1}{c}{0.38±0.06} &
  \multicolumn{1}{c}{20.50±3.29} &
  \multicolumn{1}{c}{0.53±0.01} &
  \multicolumn{1}{c}{0.71±0.03} &
  \pmb{1.00} \\ \hline
ProteinWeaver-pretrain &
  \multicolumn{1}{c}{0.69±0.18} &
  \multicolumn{1}{c}{8.79±5.74} &
  \multicolumn{1}{c}{0.74±0.13} &
  \multicolumn{1}{c}{0.69±0.06} &
  0.76 &
  \multicolumn{1}{c}{0.54±0.12} &
  \multicolumn{1}{c}{12.87±4.87} &
  \multicolumn{1}{c}{0.69±0.08} &
  \multicolumn{1}{c}{0.67±0.07} &
  0.73 \\ \hline
ProteinWeaver-sft &
  \multicolumn{1}{c}{0.66±0.16} &
  \multicolumn{1}{c}{9.71±5.61} &
  \multicolumn{1}{c}{0.70±0.13} &
  \multicolumn{1}{c}{0.69±0.05} &
  0.79 &
  \multicolumn{1}{c}{0.28±0.16} &
  \multicolumn{1}{c}{31.73±13.14} &
  \multicolumn{1}{c}{0.57±0.06} &
  \multicolumn{1}{c}{0.67±0.04} &
  0.95 \\ \hline
ProteinWeaver-sppo &
  \multicolumn{1}{c}{0.72±0.15} &
  \multicolumn{1}{c}{5.12±5.19} &
  \multicolumn{1}{c}{0.73±0.12} &
  \multicolumn{1}{c}{0.68±0.07} &
  0.75 &
  \multicolumn{1}{c}{0.63±0.13} &
  \multicolumn{1}{c}{9.17±5.81} &
  \multicolumn{1}{c}{0.69±0.10} &
  \multicolumn{1}{c}{0.68±0.06} &
  0.73 \\ \hline
ProteinWeaver-sppo (bo3) &
  \multicolumn{1}{c}{\pmb{0.79±0.12}} &
  \multicolumn{1}{c}{\pmb{4.95±3.44}} &
  \multicolumn{1}{c}{\pmb{0.78±0.12}} &
  \multicolumn{1}{c}{0.68±0.07} &
  0.76 &
  \multicolumn{1}{c}{\pmb{0.68±0.11}} &
  \multicolumn{1}{c}{\pmb{8.72±4.60}} &
  \multicolumn{1}{c}{\pmb{0.72±0.10}} &
  \multicolumn{1}{c}{0.67±0.06} &
  0.73 \\ 

  
\bottomrule
\end{tabular}
}
\end{table}

